HAT-P-58b -- HAT-P-64b: Seven Planets Transiting Bright Stars

We report the discovery and characterization of 7 transiting exoplanets from the HATNet survey. The planets, which are hot Jupiters and Saturns transiting bright sun-like stars, include: HAT-P-58b (with mass Mp = 0.37 MJ, radius Rp = 1.33 RJ, and orbital period P = 4.0138 days), HAT-P-59b (Mp = 1.54 MJ, Rp = 1.12 RJ, P = 4.1420 days), HAT-P-60b (Mp = 0.57 MJ, Rp = 1.63 RJ, P = 4.7948 days), HAT-P-61b (Mp = 1.06 MJ, Rp = 0.90 RJ, P = 1.9023 days), HAT-P-62b (Mp = 0.76 MJ, Rp = 1.07 RJ, P = 2.6453 days), HAT-P-63b (Mp = 0.61 MJ, Rp = 1.12 RJ, P = 3.3777 days), and HAT-P-64b (Mp = 0.58 MJ, Rp = 1.70 RJ, P = 4.0072 days). The typical errors on these quantities are 0.06 MJ, 0.03 RJ, and 0.2seconds, respectively. We also provide accurate stellar parameters for each of the hosts stars. With V = 9.710+/-0.050mag, HAT-P-60 is an especially bright transiting planet host, and an excellent target for additional follow-up observations. With Rp = 1.703+/-0.070 RJ, HAT-P-64b is a highly inflated hot Jupiter around a star nearing the end of its main-sequence lifetime, and is among the largest known planets. Five of the seven systems have long-cadence observations by TESS which are included in the analysis. Of particular note is HAT-P-59 (TOI-1826.01) which is within the Northern continuous viewing zone of the TESS mission, and HAT-P-60, which is the TESS candidate TOI-1580.01.

==> HTR062-011_rvtable.tex <==
HAT-P-58 & $ 6890.12499 $ & $    40.53 $ & $     7.42 $ & $   33.5 $ & $   20.2 $ & $ 0.172 $ &$   0.686 $ & HIRES \\
HAT-P-58 & $ 6892.12712 $ & $   -46.48 $ & $     2.99 $ & $  -16.9 $ & $    9.8 $ & $ 0.153 $ &$   0.185 $ & HIRES \\
HAT-P-58 & $ 6894.09295 $ & $    36.41 $ & $     2.71 $ & $   -4.2 $ & $    3.1 $ & $ 0.144 $ &$   0.675 $ & HIRES \\
HAT-P-58 & $ 6895.09290 $ & \nodata      & \nodata      & $  -15.5 $ & $    4.7 $ & $ 0.145 $ &$   0.924 $ & HIRES \\
HAT-P-58 & $ 6896.07796 $ & $   -37.36 $ & $     2.87 $ & $  -14.6 $ & $    5.6 $ & $ 0.142 $ &$   0.169 $ & HIRES \\
HAT-P-58 & $ 6909.10189 $ & $   -20.66 $ & $     3.83 $ & $   13.6 $ & $   15.5 $ & $ 0.157 $ &$   0.414 $ & HIRES \\
HAT-P-58 & $ 6910.07872 $ & $    54.59 $ & $     4.93 $ & $   24.4 $ & $   48.1 $ & $ 0.145 $ &$   0.657 $ & HIRES \\
HAT-P-58 & $ 6912.08980 $ & $   -36.75 $ & $     2.87 $ & $  -20.4 $ & $    8.0 $ & $ 0.143 $ &$   0.158 $ & HIRES \\


==> HTR080-003_rvtable.tex <==
HAT-P-59 & $ 6581.71540 $ & $  -173.34 $ & $    30.32 $ & $   -8.1 $ & $   16.1 $ & $   0.248 $ & TRES \\
HAT-P-59 & $ 6583.69510 $ & $   222.45 $ & $    26.21 $ & $   14.5 $ & $    9.7 $ & $   0.726 $ & TRES \\
HAT-P-59 & $ 6585.65905 $ & $  -166.02 $ & $    31.64 $ & $    4.4 $ & $    9.3 $ & $   0.200 $ & TRES \\
HAT-P-59 & $ 6593.29170 $ & $   -42.34 $ & $    11.50 $ & $  -48.7 $ & $   22.9 $ & $   0.043 $ & Sophie \\
HAT-P-59 & $ 6595.25025 $ & $    51.96 $ & $    36.10 $ & $ -136.2 $ & $   72.2 $ & $   0.516 $ & Sophie \\
HAT-P-59 & $ 6596.25559 $ & $   214.46 $ & $    14.70 $ & $  -12.8 $ & $   29.5 $ & $   0.759 $ & Sophie \\
HAT-P-59 & $ 6597.24301 $ & $    -6.84 $ & $     9.70 $ & $  -44.5 $ & $   19.5 $ & $   0.997 $ & Sophie \\
HAT-P-59 & $ 6598.26817 $ & $  -164.04 $ & $    31.80 $ & $  -50.0 $ & $   63.6 $ & $   0.244 $ & Sophie \\
HAT-P-59 & $ 6599.25285 $ & $   -31.24 $ & $    12.00 $ & $  -22.5 $ & $   24.0 $ & $   0.482 $ & Sophie \\
HAT-P-59 & $ 6599.26717 $ & $   -32.54 $ & $    21.10 $ & $  -81.7 $ & $   42.1 $ & $   0.486 $ & Sophie \\
HAT-P-59 & $ 6600.23567 $ & $   218.06 $ & $    21.10 $ & $   46.2 $ & $   42.2 $ & $   0.719 $ & Sophie \\
HAT-P-59 & $ 6601.31614 $ & $    27.36 $ & $     9.30 $ & $  -29.2 $ & $   18.5 $ & $   0.980 $ & Sophie \\
HAT-P-59 & $ 6602.30141 $ & $  -195.44 $ & $    14.40 $ & $  -15.3 $ & $   28.8 $ & $   0.218 $ & Sophie \\
HAT-P-59 & $ 6605.60024 $ & $   -49.83 $ & $    19.04 $ & $  -27.6 $ & $    7.9 $ & $   0.015 $ & TRES \\
HAT-P-59 & $ 6606.60413 $ & $  -152.84 $ & $    24.81 $ & $   -3.4 $ & $   24.4 $ & $   0.257 $ & TRES \\
HAT-P-59 & $ 6607.59892 $ & $   -19.99 $ & $    19.87 $ & $    0.8 $ & $   11.9 $ & $   0.497 $ & TRES \\
HAT-P-59 & $ 6608.60682 $ & $   190.72 $ & $    31.37 $ & $   -4.0 $ & $   13.8 $ & $   0.740 $ & TRES \\
HAT-P-59 & $ 6609.61035 $ & $    27.93 $ & $    18.27 $ & $   31.0 $ & $   13.6 $ & $   0.983 $ & TRES \\
HAT-P-59 & $ 6610.62724 $ & $  -214.20 $ & $    26.99 $ & $   23.6 $ & $   10.3 $ & $   0.228 $ & TRES \\
HAT-P-59 & $ 6611.59706 $ & $    -3.09 $ & $    21.75 $ & $   18.0 $ & $   17.5 $ & $   0.462 $ & TRES \\
HAT-P-59 & $ 6615.58195 $ & $  -114.55 $ & $    21.68 $ & $   -1.0 $ & $    9.4 $ & $   0.425 $ & TRES \\
HAT-P-59 & $ 6616.59129 $ & $   144.92 $ & $    12.85 $ & $  -19.8 $ & $   11.0 $ & $   0.668 $ & TRES \\
HAT-P-59 & $ 6617.62764 $ & $    62.24 $ & $    12.85 $ & $  -28.4 $ & $   10.4 $ & $   0.918 $ & TRES \\


==> HTR089-018_rvtable.tex <==
HAT-P-60 & $ 6326.58810 $ & $    42.15 $ & $    24.93 $ & $  -18.2 $ & $   15.9 $ & \nodata      & $   0.716 $ & TRES \\
HAT-P-60 & $ 6549.78555 $ & $   -57.10 $ & $    47.30 $ & $   24.4 $ & $   31.6 $ & \nodata      & $   0.266 $ & TRES \\
HAT-P-60 & $ 6551.82293 $ & $    23.30 $ & $    36.39 $ & $   44.7 $ & $   35.9 $ & \nodata      & $   0.691 $ & TRES \\
HAT-P-60 & $ 6558.92278 $ & $   -32.08 $ & $    34.84 $ & $  -51.5 $ & $   28.6 $ & \nodata      & $   0.172 $ & TRES \\
HAT-P-60 & $ 6573.89597 $ & $   -44.23 $ & $    19.98 $ & $   15.3 $ & $   10.0 $ & \nodata      & $   0.295 $ & TRES \\
HAT-P-60 & $ 6574.90009 $ & $   -41.76 $ & $    24.66 $ & $    4.4 $ & $   14.1 $ & \nodata      & $   0.504 $ & TRES \\
HAT-P-60 & $ 6575.79583 $ & $    38.08 $ & $    23.17 $ & $  -16.4 $ & $   15.2 $ & \nodata      & $   0.691 $ & TRES \\
HAT-P-60 & $ 6576.77948 $ & $     9.39 $ & $    24.46 $ & $   -1.6 $ & $   17.9 $ & \nodata      & $   0.896 $ & TRES \\
HAT-P-60 & $ 6577.80537 $ & $   -33.50 $ & $    24.93 $ & $   -3.6 $ & $   31.4 $ & \nodata      & $   0.110 $ & TRES \\
HAT-P-60 & $ 6578.74876 $ & $   -61.26 $ & $    18.25 $ & $   -7.1 $ & $   14.2 $ & \nodata      & $   0.307 $ & TRES \\
HAT-P-60 & $ 6580.72123 $ & $    66.89 $ & $    18.25 $ & $    5.2 $ & $   14.7 $ & \nodata      & $   0.718 $ & TRES \\
HAT-P-60 & $ 6581.79896 $ & $    32.21 $ & $    21.62 $ & $   13.8 $ & $   14.6 $ & \nodata      & $   0.943 $ & TRES \\
HAT-P-60 & $ 6582.85746 $ & $   -63.67 $ & $    21.79 $ & $   -9.5 $ & $   11.2 $ & \nodata      & $   0.164 $ & TRES \\
HAT-P-60 & $ 6593.49292 $ & $   -16.13 $ & $    32.40 $ & $  -82.7 $ & $   64.8 $ & \nodata      & $   0.382 $ & Sophie \\
HAT-P-60 & $ 6595.51401 $ & $    32.07 $ & $    27.10 $ & $  -54.7 $ & $   54.1 $ & \nodata      & $   0.803 $ & Sophie \\
HAT-P-60 & $ 6596.66289 $ & $   -15.03 $ & $    22.50 $ & $   28.5 $ & $   45.0 $ & \nodata      & $   0.043 $ & Sophie \\
HAT-P-60 & $ 6597.40379 $ & $   -27.23 $ & $    22.30 $ & $  -23.5 $ & $   44.6 $ & \nodata      & $   0.197 $ & Sophie \\
HAT-P-60 & $ 6599.55850 $ & $    35.07 $ & $    14.40 $ & $  -74.3 $ & $   28.8 $ & \nodata      & $   0.647 $ & Sophie \\
HAT-P-60 & $ 6600.53433 $ & $    45.07 $ & $    26.20 $ & $  -38.2 $ & $   52.3 $ & \nodata      & $   0.850 $ & Sophie \\
HAT-P-60 & $ 6601.63510 $ & $   -28.93 $ & $    22.50 $ & $   15.5 $ & $   45.0 $ & \nodata      & $   0.080 $ & Sophie \\
HAT-P-60 & $ 6602.40299 $ & $   -67.13 $ & $    15.10 $ & $  -10.2 $ & $   30.2 $ & \nodata      & $   0.240 $ & Sophie \\
HAT-P-60 & $ 6637.75333 $ & $    29.51 $ & $     3.22 $ & $    6.3 $ & $    3.2 $ & $ 0.121 $ &$   0.613 $ & HIRES \\
HAT-P-60 & $ 6638.81890 $ & $    33.03 $ & $     4.25 $ & $    0.3 $ & $    2.8 $ & $ 0.123 $ &$   0.835 $ & HIRES \\
HAT-P-60 & $ 7353.80988 $ & $    36.33 $ & $     4.11 $ & $   -8.1 $ & $    5.4 $ & $ 0.124 $ &$   0.954 $ & HIRES \\
HAT-P-60 & $ 7354.79800 $ & $   -40.93 $ & $     3.99 $ & $    8.4 $ & $    4.5 $ & $ 0.124 $ &$   0.160 $ & HIRES \\
HAT-P-60 & $ 7355.79193 $ & $   -21.46 $ & $     3.78 $ & $   -0.8 $ & $    3.7 $ & $ 0.123 $ &$   0.367 $ & HIRES \\
HAT-P-60 & $ 7355.89024 $ & \nodata      & \nodata      & $   -7.1 $ & $    4.1 $ & $ 0.122 $ &$   0.387 $ & HIRES \\
HAT-P-60 & $ 7378.72938 $ & $   -26.21 $ & $     4.10 $ & $   -0.3 $ & $    3.6 $ & $ 0.126 $ &$   0.151 $ & HIRES \\
HAT-P-60 & $ 7401.88232 $ & $    22.14 $ & $     4.50 $ & $   10.4 $ & $    4.5 $ & $ 0.121 $ &$   0.980 $ & HIRES \\
HAT-P-60 & $ 7412.79458 $ & $   -58.33 $ & $     4.40 $ & $   -9.1 $ & $    3.5 $ & $ 0.128 $ &$   0.255 $ & HIRES \\


==> HTR094-024_rvtable.tex <==
HAT-P-61 & $ 6910.98025 $ & $   149.18 $ & $    26.04 $ & $   76.1 $ & $   25.9 $ & \nodata      & $   0.743 $ & TRES \\
HAT-P-61 & $ 6911.92592 $ & $  -134.70 $ & $    33.23 $ & $   64.2 $ & $   42.9 $ & \nodata      & $   0.241 $ & TRES \\
HAT-P-61 & $ 6912.96888 $ & $   129.17 $ & $    17.84 $ & $    2.4 $ & $   28.1 $ & \nodata      & $   0.789 $ & TRES \\
HAT-P-61 & $ 6931.91154 $ & $   176.60 $ & $    27.60 $ & $  -32.9 $ & $   22.0 $ & \nodata      & $   0.747 $ & TRES \\
HAT-P-61 & $ 6932.88321 $ & $   -72.55 $ & $    36.71 $ & $  -27.9 $ & $   78.9 $ & \nodata      & $   0.257 $ & TRES \\
HAT-P-61 & $ 6934.95150 $ & $  -208.83 $ & $    17.84 $ & $  -47.2 $ & $   37.0 $ & \nodata      & $   0.345 $ & TRES \\
HAT-P-61 & $ 6935.94714 $ & $   111.18 $ & $    31.50 $ & $ -108.5 $ & $   29.2 $ & \nodata      & $   0.868 $ & TRES \\
HAT-P-61 & $ 6944.99515 $ & $   149.97 $ & $    22.95 $ & $   19.2 $ & $   24.9 $ & \nodata      & $   0.624 $ & TRES \\
HAT-P-61 & $ 6945.92201 $ & $  -161.35 $ & $    32.35 $ & $    3.7 $ & $   54.5 $ & \nodata      & $   0.112 $ & TRES \\
HAT-P-61 & $ 6958.94233 $ & $    25.21 $ & $    19.23 $ & $    3.0 $ & $   24.8 $ & \nodata      & $   0.956 $ & TRES \\
HAT-P-61 & $ 6960.00651 $ & $     2.01 $ & $    29.22 $ & $  -22.6 $ & $   39.3 $ & \nodata      & $   0.515 $ & TRES \\
HAT-P-61 & $ 6960.95084 $ & $   -69.03 $ & $    36.34 $ & $  -68.0 $ & $   42.7 $ & \nodata      & $   0.012 $ & TRES \\
HAT-P-61 & $ 6961.93882 $ & $    73.86 $ & $    35.83 $ & $   11.5 $ & $   41.9 $ & \nodata      & $   0.531 $ & TRES \\
HAT-P-61 & $ 6965.93914 $ & $   146.95 $ & $    20.19 $ & $  -15.7 $ & $   19.3 $ & \nodata      & $   0.634 $ & TRES \\
HAT-P-61 & $ 6970.92528 $ & $   -64.93 $ & $    35.63 $ & $   90.8 $ & $   23.4 $ & \nodata      & $   0.255 $ & TRES \\
HAT-P-61 & $ 6971.87773 $ & $   232.02 $ & $    31.09 $ & $   76.8 $ & $   42.3 $ & \nodata      & $   0.756 $ & TRES \\
HAT-P-61 & $ 6973.00690 $ & $   -92.82 $ & $    40.13 $ & $   -9.2 $ & $   32.6 $ & \nodata      & $   0.349 $ & TRES \\
HAT-P-61 & $ 6978.94963 $ & $   -64.74 $ & $    25.97 $ & $  -15.7 $ & $   28.7 $ & \nodata      & $   0.473 $ & TRES \\
HAT-P-61 & $ 7354.08818 $ & $   169.27 $ & $     1.12 $ & $    6.1 $ & $    8.8 $ & $ 0.258 $ &$   0.675 $ & HIRES \\
HAT-P-61 & $ 7355.08733 $ & $  -171.23 $ & $     0.90 $ & $   -1.5 $ & $    2.5 $ & $ 0.232 $ &$   0.200 $ & HIRES \\
HAT-P-61 & $ 7356.00551 $ & \nodata      & \nodata      & $    2.9 $ & $    4.8 $ & $ 0.232 $ &$   0.682 $ & HIRES \\
HAT-P-61 & $ 7356.11208 $ & $   170.17 $ & $     0.86 $ & $   -7.5 $ & $    4.7 $ & $ 0.237 $ &$   0.738 $ & HIRES \\


==> HTR130-001_rvtable.tex <==
HAT-P-62 & $ 6674.65588 $ & $  -126.65 $ & $    21.61 $ & $   30.9 $ & $   29.2 $ & $   0.258 $ & TRES \\
HAT-P-62 & $ 6707.64331 $ & $    88.60 $ & $    25.94 $ & $  -13.4 $ & $   27.3 $ & $   0.728 $ & TRES \\
HAT-P-62 & $ 6942.95953 $ & $   148.33 $ & $    23.82 $ & $  -47.5 $ & $   32.3 $ & $   0.683 $ & TRES \\
HAT-P-62 & $ 6945.86085 $ & $   164.72 $ & $    17.63 $ & $   11.1 $ & $   34.1 $ & $   0.780 $ & TRES \\
HAT-P-62 & $ 6958.92253 $ & $    74.01 $ & $    19.07 $ & $  -15.2 $ & $   18.8 $ & $   0.718 $ & TRES \\
HAT-P-62 & $ 6959.99100 $ & $   -30.23 $ & $    26.36 $ & $    1.3 $ & $   27.9 $ & $   0.121 $ & TRES \\
HAT-P-62 & $ 6960.93014 $ & $    -1.99 $ & $    20.56 $ & $  -15.8 $ & $   20.6 $ & $   0.476 $ & TRES \\
HAT-P-62 & $ 6961.91630 $ & $    33.97 $ & $    16.43 $ & $   24.2 $ & $   21.0 $ & $   0.849 $ & TRES \\
HAT-P-62 & $ 6962.86334 $ & $  -108.71 $ & $    17.73 $ & $   52.5 $ & $   24.9 $ & $   0.207 $ & TRES \\
HAT-P-62 & $ 6965.87438 $ & $  -126.58 $ & $    14.60 $ & $    0.6 $ & $   24.2 $ & $   0.346 $ & TRES \\
HAT-P-62 & $ 6970.87354 $ & $   -45.58 $ & $    22.84 $ & $  -75.3 $ & $   48.3 $ & $   0.235 $ & TRES \\
HAT-P-62 & $ 6971.83494 $ & $    56.80 $ & $    18.00 $ & $    5.3 $ & $   24.7 $ & $   0.599 $ & TRES \\
HAT-P-62 & $ 6972.87045 $ & $     2.71 $ & $    23.65 $ & $  -30.3 $ & $   23.0 $ & $   0.990 $ & TRES \\
HAT-P-62 & $ 6977.88426 $ & $    84.76 $ & $    27.25 $ & $   52.8 $ & $   26.9 $ & $   0.886 $ & TRES \\
HAT-P-62 & $ 6978.92626 $ & $  -134.32 $ & $    14.60 $ & $   18.9 $ & $   25.0 $ & $   0.279 $ & TRES \\


==> HTR384-014_phfu_tab.tex <==
HAT-P-63 & $ 56365.92055 $ & $   0.00036 $ & $   0.00172 $ & $  12.17640 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92154 $ & $   0.00034 $ & $   0.00172 $ & $  12.17370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92253 $ & $  -0.00368 $ & $   0.00172 $ & $  12.17040 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92351 $ & $   0.00099 $ & $   0.00175 $ & $  12.17740 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92448 $ & $  -0.00130 $ & $   0.00169 $ & $  12.17160 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92547 $ & $   0.00448 $ & $   0.00170 $ & $  12.17910 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92644 $ & $   0.00444 $ & $   0.00171 $ & $  12.17930 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92742 $ & $  -0.00033 $ & $   0.00170 $ & $  12.17390 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92841 $ & $  -0.00126 $ & $   0.00169 $ & $  12.17300 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.92938 $ & $   0.00235 $ & $   0.00172 $ & $  12.17810 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93038 $ & $  -0.00176 $ & $   0.00171 $ & $  12.17260 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93137 $ & $   0.00345 $ & $   0.00170 $ & $  12.17860 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93233 $ & $  -0.00559 $ & $   0.00169 $ & $  12.16850 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93332 $ & $  -0.00115 $ & $   0.00170 $ & $  12.17300 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93431 $ & $  -0.00376 $ & $   0.00169 $ & $  12.17070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93526 $ & $  -0.00047 $ & $   0.00170 $ & $  12.17360 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93622 $ & $  -0.00047 $ & $   0.00173 $ & $  12.17450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93721 $ & $   0.00025 $ & $   0.00169 $ & $  12.17470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93819 $ & $   0.00042 $ & $   0.00167 $ & $  12.17450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.93917 $ & $  -0.00151 $ & $   0.00171 $ & $  12.17290 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94017 $ & $  -0.00218 $ & $   0.00169 $ & $  12.17200 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94115 $ & $  -0.00063 $ & $   0.00169 $ & $  12.17320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94211 $ & $  -0.00309 $ & $   0.00170 $ & $  12.17170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94309 $ & $   0.00147 $ & $   0.00173 $ & $  12.17610 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94406 $ & $   0.00248 $ & $   0.00171 $ & $  12.17590 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94503 $ & $   0.00107 $ & $   0.00169 $ & $  12.17500 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94600 $ & $  -0.00107 $ & $   0.00168 $ & $  12.17230 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94697 $ & $   0.00329 $ & $   0.00169 $ & $  12.17770 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94797 $ & $   0.00366 $ & $   0.00170 $ & $  12.17780 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94895 $ & $   0.00085 $ & $   0.00167 $ & $  12.17350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.94995 $ & $   0.00025 $ & $   0.00168 $ & $  12.17380 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95092 $ & $   0.00016 $ & $   0.00165 $ & $  12.17350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95192 $ & $  -0.00102 $ & $   0.00168 $ & $  12.17320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95290 $ & $   0.00535 $ & $   0.00167 $ & $  12.17870 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95390 $ & $   0.00098 $ & $   0.00168 $ & $  12.17360 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95487 $ & $  -0.00077 $ & $   0.00169 $ & $  12.17220 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95584 $ & $  -0.00038 $ & $   0.00169 $ & $  12.17450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95683 $ & $   0.00109 $ & $   0.00168 $ & $  12.17280 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95780 $ & $  -0.00238 $ & $   0.00166 $ & $  12.16940 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95876 $ & $  -0.00190 $ & $   0.00168 $ & $  12.17000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.95975 $ & $   0.00248 $ & $   0.00168 $ & $  12.17430 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96071 $ & $  -0.00354 $ & $   0.00167 $ & $  12.16940 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96169 $ & $   0.00030 $ & $   0.00165 $ & $  12.17380 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96266 $ & $  -0.00088 $ & $   0.00166 $ & $  12.17400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96364 $ & $   0.00255 $ & $   0.00166 $ & $  12.17670 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96466 $ & $   0.00133 $ & $   0.00167 $ & $  12.17490 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96565 $ & $  -0.00028 $ & $   0.00164 $ & $  12.17260 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96661 $ & $  -0.00005 $ & $   0.00164 $ & $  12.17400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96757 $ & $  -0.00014 $ & $   0.00165 $ & $  12.17370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96853 $ & $   0.00160 $ & $   0.00170 $ & $  12.17590 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.96950 $ & $  -0.00066 $ & $   0.00165 $ & $  12.17290 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97047 $ & $  -0.00209 $ & $   0.00166 $ & $  12.17180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97146 $ & $   0.00024 $ & $   0.00165 $ & $  12.17430 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97244 $ & $  -0.00339 $ & $   0.00166 $ & $  12.17050 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97340 $ & $  -0.00054 $ & $   0.00167 $ & $  12.17420 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97438 $ & $   0.00161 $ & $   0.00164 $ & $  12.17400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97537 $ & $  -0.00016 $ & $   0.00166 $ & $  12.17380 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97634 $ & $   0.00128 $ & $   0.00168 $ & $  12.17540 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97731 $ & $   0.00234 $ & $   0.00164 $ & $  12.17670 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97831 $ & $  -0.00246 $ & $   0.00165 $ & $  12.17060 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.97929 $ & $  -0.00061 $ & $   0.00167 $ & $  12.17180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98025 $ & $  -0.00235 $ & $   0.00165 $ & $  12.17100 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98123 $ & $   0.00202 $ & $   0.00165 $ & $  12.17470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98221 $ & $  -0.00285 $ & $   0.00164 $ & $  12.17020 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98319 $ & $  -0.00090 $ & $   0.00167 $ & $  12.17190 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98417 $ & $  -0.00226 $ & $   0.00166 $ & $  12.17020 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98516 $ & $   0.00076 $ & $   0.00164 $ & $  12.17360 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98610 $ & $  -0.00089 $ & $   0.00166 $ & $  12.17200 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98710 $ & $   0.00131 $ & $   0.00165 $ & $  12.17460 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98808 $ & $  -0.00386 $ & $   0.00163 $ & $  12.16990 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.98909 $ & $   0.00019 $ & $   0.00164 $ & $  12.17250 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99007 $ & $  -0.00397 $ & $   0.00162 $ & $  12.16890 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99105 $ & $   0.00096 $ & $   0.00164 $ & $  12.17350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99201 $ & $   0.00128 $ & $   0.00163 $ & $  12.17370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99299 $ & $   0.00129 $ & $   0.00165 $ & $  12.17350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99396 $ & $  -0.00205 $ & $   0.00162 $ & $  12.16970 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99492 $ & $  -0.00050 $ & $   0.00164 $ & $  12.17210 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99588 $ & $   0.00249 $ & $   0.00164 $ & $  12.17520 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99684 $ & $   0.00221 $ & $   0.00163 $ & $  12.17490 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99781 $ & $   0.00218 $ & $   0.00165 $ & $  12.17460 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99881 $ & $   0.00608 $ & $   0.00164 $ & $  12.17840 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56365.99980 $ & $   0.00130 $ & $   0.00164 $ & $  12.17400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00078 $ & $   0.00767 $ & $   0.00164 $ & $  12.18030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00176 $ & $   0.00825 $ & $   0.00163 $ & $  12.18050 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00272 $ & $   0.00496 $ & $   0.00164 $ & $  12.17790 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00372 $ & $   0.01014 $ & $   0.00164 $ & $  12.18320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00470 $ & $   0.00891 $ & $   0.00163 $ & $  12.18070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00569 $ & $   0.00965 $ & $   0.00164 $ & $  12.18200 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00667 $ & $   0.01472 $ & $   0.00165 $ & $  12.18680 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00763 $ & $   0.01594 $ & $   0.00166 $ & $  12.18930 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00860 $ & $   0.01176 $ & $   0.00164 $ & $  12.18480 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.00960 $ & $   0.01204 $ & $   0.00164 $ & $  12.18490 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01058 $ & $   0.01146 $ & $   0.00162 $ & $  12.18450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01153 $ & $   0.01510 $ & $   0.00163 $ & $  12.18760 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01250 $ & $   0.01629 $ & $   0.00165 $ & $  12.18960 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01349 $ & $   0.01262 $ & $   0.00165 $ & $  12.18640 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01447 $ & $   0.01878 $ & $   0.00162 $ & $  12.19240 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01543 $ & $   0.01746 $ & $   0.00166 $ & $  12.19180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01642 $ & $   0.01483 $ & $   0.00163 $ & $  12.18890 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01741 $ & $   0.02025 $ & $   0.00164 $ & $  12.19430 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01839 $ & $   0.01758 $ & $   0.00165 $ & $  12.19240 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.01935 $ & $   0.01734 $ & $   0.00166 $ & $  12.19200 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02035 $ & $   0.01513 $ & $   0.00166 $ & $  12.19010 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02133 $ & $   0.01840 $ & $   0.00168 $ & $  12.19310 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02229 $ & $   0.01503 $ & $   0.00165 $ & $  12.18900 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02327 $ & $   0.01742 $ & $   0.00170 $ & $  12.19220 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02425 $ & $   0.01751 $ & $   0.00170 $ & $  12.19250 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02525 $ & $   0.01285 $ & $   0.00171 $ & $  12.18770 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02622 $ & $   0.01536 $ & $   0.00176 $ & $  12.19030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02720 $ & $   0.01768 $ & $   0.00180 $ & $  12.19300 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56366.02819 $ & $   0.01669 $ & $   0.00190 $ & $  12.19150 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.87990 $ & $   0.00044 $ & $   0.00125 $ & $  12.16930 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.88193 $ & $  -0.00172 $ & $   0.00126 $ & $  12.16710 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.88395 $ & $   0.00095 $ & $   0.00125 $ & $  12.17070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.88597 $ & $  -0.00096 $ & $   0.00125 $ & $  12.16780 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.88800 $ & $   0.00353 $ & $   0.00125 $ & $  12.17240 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.89002 $ & $   0.00762 $ & $   0.00126 $ & $  12.17820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.89204 $ & $   0.00687 $ & $   0.00124 $ & $  12.17570 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.89406 $ & $   0.01171 $ & $   0.00124 $ & $  12.18070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.89608 $ & $   0.01011 $ & $   0.00120 $ & $  12.17900 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.89812 $ & $   0.01392 $ & $   0.00123 $ & $  12.18370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.90013 $ & $   0.01446 $ & $   0.00122 $ & $  12.18390 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.90216 $ & $   0.01669 $ & $   0.00121 $ & $  12.18630 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.90417 $ & $   0.01407 $ & $   0.00124 $ & $  12.18440 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.90619 $ & $   0.01431 $ & $   0.00122 $ & $  12.18430 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.90819 $ & $   0.01822 $ & $   0.00125 $ & $  12.18820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.91019 $ & $   0.01754 $ & $   0.00122 $ & $  12.18800 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.91221 $ & $   0.01765 $ & $   0.00123 $ & $  12.18830 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.91419 $ & $   0.01806 $ & $   0.00124 $ & $  12.18780 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.91621 $ & $   0.01639 $ & $   0.00122 $ & $  12.18730 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.91824 $ & $   0.01805 $ & $   0.00127 $ & $  12.18810 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.92023 $ & $   0.01686 $ & $   0.00124 $ & $  12.18780 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.92225 $ & $   0.02046 $ & $   0.00122 $ & $  12.19100 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.92427 $ & $   0.01747 $ & $   0.00122 $ & $  12.18820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.92630 $ & $   0.01757 $ & $   0.00125 $ & $  12.18880 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.92832 $ & $   0.02256 $ & $   0.00123 $ & $  12.19260 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.93033 $ & $   0.01783 $ & $   0.00123 $ & $  12.18800 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.93235 $ & $   0.01982 $ & $   0.00120 $ & $  12.18960 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.93437 $ & $   0.02007 $ & $   0.00120 $ & $  12.19020 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.93635 $ & $   0.01812 $ & $   0.00120 $ & $  12.18770 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.93838 $ & $   0.02094 $ & $   0.00118 $ & $  12.19000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.94039 $ & $   0.01750 $ & $   0.00119 $ & $  12.18720 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.94242 $ & $   0.01929 $ & $   0.00121 $ & $  12.18820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.94444 $ & $   0.01984 $ & $   0.00121 $ & $  12.19000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.94648 $ & $   0.01787 $ & $   0.00120 $ & $  12.19010 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.94846 $ & $   0.01771 $ & $   0.00120 $ & $  12.18760 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.95048 $ & $   0.01606 $ & $   0.00121 $ & $  12.18740 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.95251 $ & $   0.01827 $ & $   0.00120 $ & $  12.18840 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.95457 $ & $   0.02065 $ & $   0.00122 $ & $  12.19140 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.95659 $ & $   0.01872 $ & $   0.00121 $ & $  12.18960 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.95862 $ & $   0.01700 $ & $   0.00121 $ & $  12.18790 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.96064 $ & $   0.01839 $ & $   0.00121 $ & $  12.18890 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.96264 $ & $   0.01715 $ & $   0.00120 $ & $  12.18770 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.96468 $ & $   0.01594 $ & $   0.00118 $ & $  12.18610 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.96669 $ & $   0.01615 $ & $   0.00117 $ & $  12.18470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.96873 $ & $   0.01717 $ & $   0.00121 $ & $  12.18620 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.97074 $ & $   0.01746 $ & $   0.00121 $ & $  12.18590 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.97274 $ & $   0.01622 $ & $   0.00120 $ & $  12.18450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.97478 $ & $   0.01559 $ & $   0.00119 $ & $  12.18400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.97679 $ & $   0.01463 $ & $   0.00120 $ & $  12.18260 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.97883 $ & $   0.01807 $ & $   0.00121 $ & $  12.18670 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.98083 $ & $   0.01380 $ & $   0.00120 $ & $  12.18220 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.98287 $ & $   0.01457 $ & $   0.00119 $ & $  12.18310 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.98489 $ & $   0.01506 $ & $   0.00119 $ & $  12.18320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.98692 $ & $   0.01186 $ & $   0.00119 $ & $  12.18030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.98894 $ & $   0.01265 $ & $   0.00118 $ & $  12.18190 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.99095 $ & $   0.01154 $ & $   0.00119 $ & $  12.18100 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.99301 $ & $   0.01055 $ & $   0.00121 $ & $  12.18050 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.99501 $ & $   0.00610 $ & $   0.00118 $ & $  12.17570 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.99705 $ & $   0.00368 $ & $   0.00115 $ & $  12.17320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56382.99907 $ & $   0.00155 $ & $   0.00116 $ & $  12.17130 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.00109 $ & $  -0.00012 $ & $   0.00119 $ & $  12.16990 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.00312 $ & $  -0.00210 $ & $   0.00117 $ & $  12.16850 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.00513 $ & $   0.00081 $ & $   0.00116 $ & $  12.17060 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.00716 $ & $  -0.00234 $ & $   0.00118 $ & $  12.16890 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.00918 $ & $   0.00140 $ & $   0.00119 $ & $  12.17170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.01121 $ & $   0.00039 $ & $   0.00119 $ & $  12.17070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.01320 $ & $   0.00127 $ & $   0.00123 $ & $  12.17170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56383.01521 $ & $  -0.00044 $ & $   0.00126 $ & $  12.17020 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.84790 $ & $   0.02013 $ & $   0.00190 $ & $  12.25890 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.84888 $ & $   0.02171 $ & $   0.00192 $ & $  12.26050 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.84984 $ & $   0.01705 $ & $   0.00187 $ & $  12.25460 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85082 $ & $   0.01882 $ & $   0.00195 $ & $  12.25640 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85181 $ & $   0.01808 $ & $   0.00199 $ & $  12.25700 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85279 $ & $   0.01464 $ & $   0.00192 $ & $  12.25350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85374 $ & $   0.01739 $ & $   0.00190 $ & $  12.25540 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85474 $ & $   0.01683 $ & $   0.00198 $ & $  12.25390 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85572 $ & $   0.02327 $ & $   0.00189 $ & $  12.26230 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85670 $ & $   0.01623 $ & $   0.00189 $ & $  12.25450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85767 $ & $   0.01925 $ & $   0.00188 $ & $  12.25630 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85863 $ & $   0.01835 $ & $   0.00195 $ & $  12.25510 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.85961 $ & $   0.02032 $ & $   0.00195 $ & $  12.25720 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86057 $ & $   0.01579 $ & $   0.00187 $ & $  12.25340 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86153 $ & $   0.01505 $ & $   0.00197 $ & $  12.24950 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86251 $ & $   0.01794 $ & $   0.00195 $ & $  12.25470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86350 $ & $   0.01611 $ & $   0.00191 $ & $  12.25380 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86449 $ & $   0.01396 $ & $   0.00194 $ & $  12.24990 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86550 $ & $   0.01976 $ & $   0.00190 $ & $  12.25810 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86645 $ & $   0.01553 $ & $   0.00186 $ & $  12.25450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86741 $ & $   0.01623 $ & $   0.00188 $ & $  12.25310 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86840 $ & $   0.01496 $ & $   0.00189 $ & $  12.25330 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.86937 $ & $   0.01336 $ & $   0.00185 $ & $  12.25030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87036 $ & $   0.01724 $ & $   0.00186 $ & $  12.25400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87136 $ & $   0.01527 $ & $   0.00189 $ & $  12.25180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87238 $ & $   0.01223 $ & $   0.00189 $ & $  12.25090 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87335 $ & $   0.01267 $ & $   0.00183 $ & $  12.25060 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87433 $ & $   0.01226 $ & $   0.00181 $ & $  12.25080 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87532 $ & $   0.01672 $ & $   0.00182 $ & $  12.25440 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87631 $ & $   0.01300 $ & $   0.00179 $ & $  12.25000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87730 $ & $   0.00885 $ & $   0.00180 $ & $  12.24640 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87829 $ & $   0.00715 $ & $   0.00179 $ & $  12.24540 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.87928 $ & $   0.00847 $ & $   0.00178 $ & $  12.24760 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88025 $ & $   0.00716 $ & $   0.00181 $ & $  12.24470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88121 $ & $   0.01047 $ & $   0.00181 $ & $  12.24770 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88218 $ & $   0.00638 $ & $   0.00180 $ & $  12.24560 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88316 $ & $   0.00544 $ & $   0.00184 $ & $  12.24310 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88415 $ & $   0.00803 $ & $   0.00179 $ & $  12.24600 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88511 $ & $   0.00310 $ & $   0.00184 $ & $  12.24080 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88608 $ & $   0.00289 $ & $   0.00180 $ & $  12.24040 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88708 $ & $   0.00309 $ & $   0.00177 $ & $  12.24080 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88806 $ & $  -0.00074 $ & $   0.00174 $ & $  12.23710 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.88903 $ & $  -0.00515 $ & $   0.00173 $ & $  12.23370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89002 $ & $   0.00018 $ & $   0.00176 $ & $  12.23840 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89099 $ & $   0.00085 $ & $   0.00175 $ & $  12.24010 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89195 $ & $   0.00242 $ & $   0.00178 $ & $  12.24040 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89291 $ & $   0.00545 $ & $   0.00187 $ & $  12.24310 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89388 $ & $   0.00057 $ & $   0.00176 $ & $  12.24080 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89486 $ & $   0.00155 $ & $   0.00178 $ & $  12.23750 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89584 $ & $   0.00265 $ & $   0.00175 $ & $  12.24190 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89681 $ & $  -0.00268 $ & $   0.00174 $ & $  12.23640 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89778 $ & $   0.00200 $ & $   0.00176 $ & $  12.24180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89877 $ & $   0.00071 $ & $   0.00177 $ & $  12.24030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.89973 $ & $  -0.00040 $ & $   0.00170 $ & $  12.23850 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90071 $ & $   0.00303 $ & $   0.00173 $ & $  12.24220 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90171 $ & $   0.00040 $ & $   0.00172 $ & $  12.23950 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90269 $ & $   0.00364 $ & $   0.00174 $ & $  12.24250 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90365 $ & $  -0.00166 $ & $   0.00173 $ & $  12.23820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90465 $ & $  -0.00076 $ & $   0.00173 $ & $  12.24010 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90562 $ & $   0.00067 $ & $   0.00176 $ & $  12.24210 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90660 $ & $  -0.00397 $ & $   0.00175 $ & $  12.23720 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90758 $ & $   0.00186 $ & $   0.00175 $ & $  12.24400 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90854 $ & $  -0.00095 $ & $   0.00173 $ & $  12.24170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.90950 $ & $  -0.00085 $ & $   0.00172 $ & $  12.24140 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91047 $ & $  -0.00099 $ & $   0.00175 $ & $  12.24100 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91144 $ & $  -0.00190 $ & $   0.00173 $ & $  12.24000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91241 $ & $  -0.00085 $ & $   0.00173 $ & $  12.24030 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91341 $ & $  -0.00123 $ & $   0.00172 $ & $  12.24060 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91437 $ & $  -0.00016 $ & $   0.00176 $ & $  12.24170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91537 $ & $   0.00117 $ & $   0.00171 $ & $  12.24240 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91634 $ & $  -0.00212 $ & $   0.00171 $ & $  12.23920 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91733 $ & $  -0.00030 $ & $   0.00172 $ & $  12.24130 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91834 $ & $  -0.00464 $ & $   0.00173 $ & $  12.23660 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.91934 $ & $  -0.00224 $ & $   0.00173 $ & $  12.23980 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92031 $ & $   0.00263 $ & $   0.00175 $ & $  12.24490 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92127 $ & $   0.00277 $ & $   0.00175 $ & $  12.24500 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92225 $ & $   0.00155 $ & $   0.00173 $ & $  12.24320 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92323 $ & $   0.00281 $ & $   0.00175 $ & $  12.24470 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92422 $ & $  -0.00070 $ & $   0.00174 $ & $  12.23990 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92517 $ & $  -0.00229 $ & $   0.00177 $ & $  12.23840 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92614 $ & $   0.00041 $ & $   0.00175 $ & $  12.24170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92713 $ & $   0.00178 $ & $   0.00172 $ & $  12.24190 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92812 $ & $  -0.00596 $ & $   0.00173 $ & $  12.23530 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.92909 $ & $  -0.00055 $ & $   0.00176 $ & $  12.24070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93009 $ & $   0.00270 $ & $   0.00178 $ & $  12.24290 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93106 $ & $  -0.00209 $ & $   0.00174 $ & $  12.23660 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93203 $ & $  -0.00103 $ & $   0.00177 $ & $  12.23970 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93301 $ & $  -0.00156 $ & $   0.00174 $ & $  12.23820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93398 $ & $   0.00070 $ & $   0.00176 $ & $  12.24120 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93496 $ & $  -0.00176 $ & $   0.00174 $ & $  12.23900 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93595 $ & $  -0.00073 $ & $   0.00175 $ & $  12.23960 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93693 $ & $  -0.00229 $ & $   0.00180 $ & $  12.23910 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93791 $ & $   0.00145 $ & $   0.00176 $ & $  12.24290 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93887 $ & $   0.00342 $ & $   0.00182 $ & $  12.24450 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.93986 $ & $  -0.00446 $ & $   0.00174 $ & $  12.23660 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94083 $ & $  -0.00125 $ & $   0.00191 $ & $  12.23970 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94182 $ & $   0.00164 $ & $   0.00179 $ & $  12.24090 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94281 $ & $   0.00367 $ & $   0.00185 $ & $  12.24340 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94378 $ & $  -0.00088 $ & $   0.00181 $ & $  12.23880 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94474 $ & $   0.00474 $ & $   0.00180 $ & $  12.24370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94570 $ & $  -0.00178 $ & $   0.00180 $ & $  12.23810 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94669 $ & $   0.00456 $ & $   0.00178 $ & $  12.24340 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94766 $ & $  -0.00356 $ & $   0.00181 $ & $  12.23500 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94866 $ & $  -0.00278 $ & $   0.00181 $ & $  12.23550 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.94965 $ & $  -0.00418 $ & $   0.00181 $ & $  12.23360 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95062 $ & $  -0.00177 $ & $   0.00189 $ & $  12.23650 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95161 $ & $   0.00062 $ & $   0.00178 $ & $  12.24020 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95257 $ & $   0.00169 $ & $   0.00192 $ & $  12.24070 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95353 $ & $  -0.00023 $ & $   0.00181 $ & $  12.23970 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95452 $ & $   0.00212 $ & $   0.00176 $ & $  12.24210 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95552 $ & $   0.00155 $ & $   0.00183 $ & $  12.24040 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95649 $ & $   0.00098 $ & $   0.00176 $ & $  12.24000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95745 $ & $   0.00275 $ & $   0.00177 $ & $  12.24130 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95843 $ & $   0.00655 $ & $   0.00181 $ & $  12.24530 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.95941 $ & $   0.00035 $ & $   0.00185 $ & $  12.23820 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96043 $ & $   0.00153 $ & $   0.00178 $ & $  12.24010 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96138 $ & $  -0.00176 $ & $   0.00176 $ & $  12.23810 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96236 $ & $   0.00339 $ & $   0.00178 $ & $  12.24370 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96331 $ & $   0.00209 $ & $   0.00173 $ & $  12.24170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96431 $ & $  -0.00014 $ & $   0.00171 $ & $  12.24100 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96529 $ & $   0.00193 $ & $   0.00172 $ & $  12.24130 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96626 $ & $   0.00144 $ & $   0.00174 $ & $  12.24140 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96724 $ & $  -0.00368 $ & $   0.00176 $ & $  12.23510 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96823 $ & $  -0.00286 $ & $   0.00171 $ & $  12.23750 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.96921 $ & $   0.00339 $ & $   0.00173 $ & $  12.24300 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97017 $ & $   0.00016 $ & $   0.00170 $ & $  12.24090 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97115 $ & $   0.00241 $ & $   0.00168 $ & $  12.24180 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97213 $ & $  -0.00152 $ & $   0.00173 $ & $  12.23700 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97310 $ & $  -0.00075 $ & $   0.00171 $ & $  12.23910 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97409 $ & $   0.00059 $ & $   0.00174 $ & $  12.23860 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97504 $ & $  -0.00005 $ & $   0.00172 $ & $  12.23910 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97603 $ & $  -0.00124 $ & $   0.00173 $ & $  12.23720 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97701 $ & $  -0.00065 $ & $   0.00174 $ & $  12.24000 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97801 $ & $   0.00110 $ & $   0.00175 $ & $  12.23970 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.97898 $ & $  -0.00093 $ & $   0.00174 $ & $  12.23790 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98000 $ & $  -0.00206 $ & $   0.00184 $ & $  12.23610 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98099 $ & $   0.00070 $ & $   0.00178 $ & $  12.23990 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98195 $ & $   0.00149 $ & $   0.00180 $ & $  12.23980 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98291 $ & $   0.00163 $ & $   0.00175 $ & $  12.23980 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98388 $ & $   0.00163 $ & $   0.00177 $ & $  12.24040 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98487 $ & $  -0.00052 $ & $   0.00174 $ & $  12.23830 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98582 $ & $   0.00152 $ & $   0.00175 $ & $  12.24110 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98680 $ & $   0.00064 $ & $   0.00175 $ & $  12.23910 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98779 $ & $  -0.00298 $ & $   0.00180 $ & $  12.23460 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98876 $ & $  -0.00320 $ & $   0.00175 $ & $  12.23490 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.98976 $ & $  -0.00309 $ & $   0.00185 $ & $  12.23350 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99073 $ & $  -0.00036 $ & $   0.00177 $ & $  12.23670 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99171 $ & $  -0.00063 $ & $   0.00181 $ & $  12.23620 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99269 $ & $   0.00406 $ & $   0.00178 $ & $  12.24170 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99366 $ & $  -0.00213 $ & $   0.00178 $ & $  12.23440 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99464 $ & $   0.00023 $ & $   0.00179 $ & $  12.23780 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99563 $ & $  -0.00098 $ & $   0.00183 $ & $  12.23760 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99662 $ & $  -0.00086 $ & $   0.00180 $ & $  12.23700 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99762 $ & $  -0.00282 $ & $   0.00181 $ & $  12.23520 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99858 $ & $   0.00324 $ & $   0.00186 $ & $  12.24090 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56399.99955 $ & $   0.00183 $ & $   0.00184 $ & $  12.23880 $ & $ i$ &  KeplerCam\\
HAT-P-63 & $ 56400.00055 $ & $  -0.00355 $ & $   0.00201 $ & $  12.23310 $ & $ i$ &  KeplerCam\\


==> HTR384-014_rvtable.tex <==
HAT-P-63 & $ 6023.91391 $ & $   129.50 $ & $    38.60 $ & $    0.0 $ & $    0.0 $ & $   0.707 $ & TRES \\
HAT-P-63 & $ 6045.89542 $ & $   -84.12 $ & $    38.60 $ & $    0.0 $ & $ -427.2 $ & $   0.215 $ & TRES \\
HAT-P-63 & $ 6189.73983 $ & \nodata      & \nodata      & $   -4.9 $ & $   19.9 $ & $   0.801 $ & HDS \\
HAT-P-63 & $ 6189.75456 $ & \nodata      & \nodata      & $   -9.9 $ & $   20.4 $ & $   0.805 $ & HDS \\
HAT-P-63 & $ 6189.76928 $ & \nodata      & \nodata      & $   -5.0 $ & $   22.9 $ & $   0.810 $ & HDS \\
HAT-P-63 & $ 6189.78400 $ & \nodata      & \nodata      & $   -9.1 $ & $   22.6 $ & $   0.814 $ & HDS \\
HAT-P-63 & $ 6190.73339 $ & $   -54.82 $ & $     7.80 $ & $   -1.0 $ & $   23.4 $ & $   0.095 $ & HDS \\
HAT-P-63 & $ 6190.74813 $ & $   -54.06 $ & $     7.84 $ & $   13.8 $ & $   18.3 $ & $   0.100 $ & HDS \\
HAT-P-63 & $ 6190.76286 $ & $   -58.71 $ & $     8.10 $ & $   10.1 $ & $   16.5 $ & $   0.104 $ & HDS \\
HAT-P-63 & $ 6190.77762 $ & $   -58.26 $ & $     7.29 $ & $    4.0 $ & $   17.5 $ & $   0.108 $ & HDS \\
HAT-P-63 & $ 6191.73872 $ & $   -53.97 $ & $    12.13 $ & $   11.2 $ & $    8.7 $ & $   0.393 $ & HDS \\
HAT-P-63 & $ 6191.75344 $ & $   -47.95 $ & $    10.48 $ & $   -7.7 $ & $    9.0 $ & $   0.397 $ & HDS \\
HAT-P-63 & $ 6191.76817 $ & $   -49.52 $ & $    13.25 $ & $   15.8 $ & $   12.8 $ & $   0.402 $ & HDS \\
HAT-P-63 & $ 6191.78289 $ & $   -62.43 $ & $    12.27 $ & $   32.1 $ & $   14.5 $ & $   0.406 $ & HDS \\
HAT-P-63 & $ 6192.73493 $ & $    79.05 $ & $     8.31 $ & $  -14.2 $ & $   18.9 $ & $   0.688 $ & HDS \\
HAT-P-63 & $ 6192.74967 $ & $    80.64 $ & $     7.60 $ & $   -4.2 $ & $   12.3 $ & $   0.692 $ & HDS \\
HAT-P-63 & $ 6192.76439 $ & $    80.82 $ & $     8.44 $ & $  -16.0 $ & $   17.3 $ & $   0.697 $ & HDS \\
HAT-P-63 & $ 6192.77911 $ & $    77.11 $ & $     8.65 $ & $  -14.9 $ & $   15.3 $ & $   0.701 $ & HDS \\
HAT-P-63 & $ 6446.51381 $ & $    54.19 $ & $    18.60 $ & $  -51.2 $ & $   37.2 $ & $   0.821 $ & Sophie \\
HAT-P-63 & $ 6447.50510 $ & $   -35.01 $ & $    12.50 $ & $   -6.5 $ & $   25.0 $ & $   0.114 $ & Sophie \\
HAT-P-63 & $ 6448.56434 $ & $   -37.31 $ & $    13.10 $ & $   -5.8 $ & $   26.2 $ & $   0.428 $ & Sophie \\
HAT-P-63 & $ 6449.56056 $ & $    45.69 $ & $    14.70 $ & $  -36.7 $ & $   29.4 $ & $   0.723 $ & Sophie \\
HAT-P-63 & $ 6451.51641 $ & $  -100.41 $ & $    11.30 $ & $  -15.0 $ & $   22.6 $ & $   0.302 $ & Sophie \\
HAT-P-63 & $ 6454.53652 $ & $   -72.61 $ & $    12.20 $ & $  -77.2 $ & $   24.4 $ & $   0.196 $ & Sophie \\
HAT-P-63 & $ 6456.50551 $ & $   103.69 $ & $     8.20 $ & $  -21.7 $ & $   16.4 $ & $   0.779 $ & Sophie \\


==> HTR405-001_rvtable.tex <==
HAT-P-64 & $ 5611.85377 $ & \nodata      & \nodata      & $   13.3 $ & $    8.1 $ & $ 0.159 $ &$   0.063 $ & HIRES \\
HAT-P-64 & $ 5611.86923 $ & $   -27.85 $ & $     8.60 $ & $    3.8 $ & $    8.4 $ & $ 0.140 $ &$   0.067 $ & HIRES \\
HAT-P-64 & $ 5815.07604 $ & $    51.41 $ & $     6.24 $ & $   -0.1 $ & $    8.1 $ & $ 0.141 $ &$   0.777 $ & HIRES \\
HAT-P-64 & $ 5815.08975 $ & \nodata      & \nodata      & $   -2.4 $ & $    6.2 $ & $ 0.140 $ &$   0.781 $ & HIRES \\
HAT-P-64 & $ 5853.92294 $ & $     5.75 $ & $     7.85 $ & $    2.3 $ & $    9.6 $ & $ 0.137 $ &$   0.471 $ & HIRES \\
HAT-P-64 & $ 5879.92287 $ & $    20.12 $ & $     6.98 $ & $   17.1 $ & $    9.6 $ & $ 0.148 $ &$   0.960 $ & HIRES \\
HAT-P-64 & $ 5882.12309 $ & $   -31.01 $ & $     8.59 $ & $  -93.6 $ & $   18.5 $ & $ 0.151 $ &$   0.509 $ & HIRES \\
HAT-P-64 & $ 5901.44866 $ & $   -93.15 $ & $    44.00 $ & $ -349.0 $ & $   88.0 $ & \nodata      & $   0.331 $ & Sophie \\
HAT-P-64 & $ 5902.42391 $ & $    50.85 $ & $    29.00 $ & $ -149.0 $ & $   58.0 $ & \nodata      & $   0.575 $ & Sophie \\
HAT-P-64 & $ 5903.49529 $ & $   104.85 $ & $    28.00 $ & $  -16.0 $ & $   56.0 $ & \nodata      & $   0.842 $ & Sophie \\
HAT-P-64 & $ 5904.47960 $ & $   -40.15 $ & $    25.00 $ & $  -15.0 $ & $   50.0 $ & \nodata      & $   0.088 $ & Sophie \\
HAT-P-64 & $ 5904.79205 $ & $   -30.84 $ & $     7.20 $ & \nodata      & \nodata      & \nodata      & $   0.166 $ & HIRES \\
HAT-P-64 & $ 5906.40764 $ & $    35.85 $ & $    29.00 $ & $  172.0 $ & $   58.0 $ & \nodata      & $   0.569 $ & Sophie \\
HAT-P-64 & $ 5908.43207 $ & $   -82.15 $ & $    33.00 $ & $  -28.0 $ & $   66.0 $ & \nodata      & $   0.074 $ & Sophie \\
HAT-P-64 & $ 5944.89703 $ & $   -73.94 $ & $     7.44 $ & $  -12.3 $ & $    9.7 $ & $ 0.145 $ &$   0.174 $ & HIRES \\

